Technical Proposal: FASERnu

FASERnu is a proposed small and inexpensive emulsion detector designed to detect collider neutrinos for the first time and study their properties. FASERnu will be located directly in front of FASER, 480 m from the ATLAS interaction point along the beam collision axis in the unused service tunnel TI12. From 2021-23 during Run 3 of the 14 TeV LHC, roughly 1,300 electron neutrinos, 20,000 muon neutrinos, and 20 tau neutrinos will interact in FASERnu with TeV-scale energies. With the ability to observe these interactions, reconstruct their energies, and distinguish flavors, FASERnu will probe the production, propagation, and interactions of neutrinos at the highest human-made energies ever recorded. The FASERnu detector will be composed of 1000 emulsion layers interleaved with tungsten plates. The total volume of the emulsion and tungsten is 25cm x 25cm x 1.35m, and the tungsten target mass is 1.2 tonnes. From 2021-23, 7 sets of emulsion layers will be installed, with replacement roughly every 20-50 1/fb in planned Technical Stops. In this document, we summarize FASERnu's physics goals and discuss the estimates of neutrino flux and interaction rates. We then describe the FASERnu detector in detail, including plans for assembly, transport, installation, and emulsion replacement, and procedures for emulsion readout and analyzing the data. We close with cost estimates for the detector components and infrastructure work and a timeline for the experiment.

==> header.tex <==

\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
%,pagecolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\bibliographystyle{utphys} % PRD-like, adds titles, %%ARXIV
\allowdisplaybreaks

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{dcolumn}	% Align table columns on decimal point
\usepackage{hyperref}      	% hypertext links %%ARXIV
\usepackage{bm}		% bold math
\usepackage{epsfig}
\usepackage{epstopdf}
\usepackage{setspace}
\usepackage[usenames, dvipsnames]{color}
\usepackage{slashed}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{siunitx}
\usepackage{multirow}
\usepackage{datetime}
\usepackage{lineno}
\usepackage{float}
\usepackage{xspace}
\usepackage{booktabs}
%\linenumbers

\newcommand{\ssection}[1]{{\em #1.\ }}
\newcommand{\PRE}[1]{{#1}} % Use if preprint style

\newcommand{\be}{\begin{equation}\begin{aligned}}
\newcommand{\ee}{\end{aligned}\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\nn}{\nonumber}

\newcommand{\gweak}{g_{\text{weak}}}
\newcommand{\mweak}{m_{\text{weak}}}
\newcommand{\mplanck}{M_{\text{Pl}}}
\newcommand{\mstar}{M_{*}}
\newcommand{\sigmaan}{\sigma_{\text{an}}}
\newcommand{\sigmatot}{\sigma_{\text{tot}}}
\newcommand{\OmegaM}{\Omega_{\text{M}}}
\newcommand{\OmegaDM}{\Omega_{\text{DM}}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\br}{\text{BR}}
\newcommand{\K}{\text{K}}
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}
\newcommand{\fb}{\text{fb}}
\newcommand{\pb}{\text{pb}}
\newcommand{\mb}{\text{mb}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}
\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}
\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\sr}{\text{sr}}
\newcommand{\fs}{\text{fs}\xspace}
\newcommand{\ps}{\text{ps}\xspace}
\newcommand{\ns}{\text{ns}\xspace}
\newcommand{\mus}{\ensuremath{\mu}\text{s}\xspace}
\newcommand{\s}{\text{s}}
\newcommand{\yr}{\text{yr}}
\newcommand{\Hz}{\text{Hz}\xspace}
\newcommand{\kHz}{\text{kHz}\xspace}
\newcommand{\MHz}{\text{MHz}\xspace}
\newcommand{\kpc}{\text{kpc}}
\newcommand{\Mpc}{\text{Mpc}}
\newcommand{\etal}{{\em et al.}}
\newcommand{\eg}{{\em e.g.}}
\newcommand{\ie}{{\em i.e.}}
\newcommand{\ibid}{{\em ibid.}}
\newcommand{\Eqref}[1]{Equation~(\ref{#1})}
\newcommand{\Eqsref}[2]{Equations~(\ref{#1}) and (\ref{#2})}
\renewcommand{\eqref}[1]{Eq.~(\ref{#1})}
\newcommand{\eqsref}[2]{Eqs.~(\ref{#1}) and (\ref{#2})}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\secsref}[2]{Secs.~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figsref}[2]{Figs.~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tableref}[1]{Table~\ref{table:#1}}
\newcommand{\tablesref}[2]{Tables~\ref{table:#1} and \ref{table:#2}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\appsref}[2]{Appendices~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\sla}[1]{\not{\! #1}}
\newcommand{\slas}[1]{\! \not{\! \! #1}}
\newcommand{\slass}[1]{\! \not{\! #1}}
%\newcommand{\gsim}{\lower.7ex\hbox{$\;\stackrel{\textstyle>}{\sim}\;$}}
%\newcommand{\lsim}{\lower.7ex\hbox{$\;\stackrel{\textstyle<}{\sim}\;$}}

\newcommand{\TAN}{TAXN}
\newcommand{\lmin}{L_{\text{min}}}
\newcommand{\lmax}{L_{\text{max}}}
\newcommand{\ltan}{L_{\text{\TAN}}}
\newcommand{\aang}{{\cal A}_{\text{ang}}}
\newcommand{\mphi}{m_{\phi}}
\newcommand{\nsig}{N_{\text{sig}}}
\newcommand{\loverlap}{\ell_{\text{overlap}}}
\newcommand{\ydown}{y_{\text{down}}}
\newcommand{\yup}{y_{\text{up}}}
\newcommand{\order}[1]{\mathcal{O}(#1)}
\newcommand{\units}[1]{\mathrm{#1}}

\newcommand{\gpi}{g_{\pi^0\gamma\gamma}}
\newcommand{\geta}{g_{\eta\gamma\gamma}}
\newcommand{\ga}{g_{a\gamma\gamma}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\black}[1]{\textcolor{black}{#1}}

\renewcommand{\abstractname}{\bf Executive Summary}

\newcommand{\rem}[1]{\textcolor{red}{[JLF: {#1}]}}
%\newcommand{\rem}[1]{\textcolor{red}{}}
\newcommand{\Felix}[1]{\textcolor{magenta}{[FK: {#1}]}}
\newcommand{\Sebastian}[1]{\textcolor{Emerald}{[ST:#1]}}
%\newcommand{\Sebastian}[1]{\textcolor{Emerald}{}}
\newcommand{\Dave}[1]{\textcolor{BurntOrange}{[DC: {#1}]}}
\newcommand{\Hide}[1]{\textcolor{Yellow}{[HO: {#1}]}}
\newcommand{\Jamie}[1]{\textcolor{Cyan}{[JB: {#1}]}}
\newcommand{\Aki}[1]{\textcolor{blue}{[AA: {#1}]}}
\newcommand{\Tomoko}[1]{\textcolor{blue}{[TA: {#1}]}}
\newcommand{\Jordan}[1]{\textcolor{TealBlue}{[JS: {#1}]}}
\newcommand{\Callum}[1]{\textcolor{blue}{[CW: {#1}]}}

\newcommand{\content}[1]{\textcolor{Gray}{Proposed Content: {#1}}}

\newcommand{\FASERnu}{FASER$\nu$\xspace}

\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}

\makeatletter
\def\l@subsubsection#1#2{}
\makeatother
